Online Set-Based Dynamic Analysis for Sound Predictive Race Detection

Predictive data race detectors find data races that exist in executions other than the observed execution. Smaragdakis et al. introduced the causally-precedes (CP) relation and a polynomial-time analysis for sound (no false races) predictive data race detection. However, their analysis cannot scale beyond analyzing bounded windows of execution traces. This work introduces a novel dynamic analysis called Raptor that computes CP soundly and completely. Raptor is inherently an online analysis that analyzes and finds all CP-races of an execution trace in its entirety. An evaluation of a prototype implementation of Raptor shows that it scales to program executions that the prior CP analysis cannot handle, finding data races that the prior CP analysis cannot find.

==> AdditionsAndComplications.tex <==
%auto-ignore
% Very old original attempt at GCP [outdated]
\section{Complications and Additions}
To be able to properly track information for locksets, separate structures
are created: \RaceSet, \GTL, \PCP, and \VC.

\subsection{\underline{G}lobal \underline{T}hread \underline{L}ock Set}
The \GTL is used to provide global information on which locks are currently held
by which threads in any given state. This information is necessary when a
variable is being accessed, to reveal otherwise hidden lock nesting, and
evaluating lock to lock dependencies such as when elements are added to the \PCP
set. The \GTL achieves providing this information by keeping a list of locks
mapped to the thread currently holding the lock. The \GTL is needed to handle
all \CP relation rules.

\subsection{RaceSet}
The \RaceSet is introduced to handle potential lazy races which arise when
\RuleB delays the information indicating a release/acquire pair form a \CP edge.
The elements within the \RaceSet take the form:
\begin{itemize}
  \item \textbf{\RaceElement{x}{m}{v}} = if \RaceElement{x}{m}{v} $\in$ \RaceSet
  then variable \code{x} was accessed a second time by a thread \code{T}
  $\notin$ \CPLockSet{x}{} while $\PCPLockSet{x}{} \neq \emptyset$.
\end{itemize}
This allows a \CP race to be delayed until no more possible \CP edges can be
established. If an element still exists within \PCPLockSet{x}{}, then the \CP
race may not be a true \CP race due to a late \CP edge being established. This
allows the second access to \code{y} in figure~\ref{tab:RuleB} to delay
reporting a race until the enclosing critical section on lock \code{m} has
released. In this example, the \CP edge from \Release{m} by \code{T1} to
\Acquire{m} by \code{T2} was delayed until the access to \code{x}, thus delaying
the knowledge of the \CP edge for variable \code{y}.
 
\subsection{\underline{P}ossibly \underline{C}ausally \underline{P}rocedes}
The \PCP set is extensively used in conjunction with the \RaceSet to provide the
necessary information of possible \CP edges formed per variable. The \PCP set
is needed for the use of \RuleC in combination with \RuleB. The elements
within the \PCP set takes the form:
\begin{itemize}
  \item \textbf{\PCPLock{n}{v}{m}{w}} = if \PCPLock{n}{v}{m}{w} $\in$
  \PCPLockSet{x}{} then \HBLock{m}{w} \HBRelation \HBLock{n}{v}. So if
  \HBLock{m}{w} established \CP from delay then \HBLock{n}{v} will also
  established \CP ordering. We also say \HBLock{n}{v} is dependent on
  \HBLock{m}{w} or \HBLock{m}{w} is providing for \HBLock{n}{v}.
\end{itemize}
Because of the composition of \RuleC, it is possible for \RuleB to lead into
\RuleC and for \RuleC to lead into \RuleB. So as one \CP edge is delayed in
establishement due to \RuleB a cascading effect can occur due to \RuleC. In
order to capture this cascading effect without looking backward in the program,
a variable keeps the \HB ordered locks which could possibly be \CP ordered in
the \PCP set. As \PCP locks are ordered to different threads by \HB or \CP
ordering, these threads are also added to the \PCP set.

The restriction on \PCP sets limit the addition of an element to be either a
nested lock or a thread ordered to by a lock element already within the \PCP
set. The next restriction on \PCP sets limits the addition of a thread element
to all orderings from a lock element within \PCP to a thread on the condition
that a lazy race for variable \code{x} of \PCPLockSet{x}{} has not been
discovered. \PCP elements are removed when either the possible \CP relation is
finally established or the providing enclosing lock finally releases.

\subsection{\underline{V}ector \underline{C}lock}
The addition of \VC is to provide information on when an \Acquire{m} by
\code{T} \CPRelation \Release{m} by \code{T`}. This function is needed primarily
by \RuleB to verify that an \Acquire{m} has a path which is \CP ordered to a
\Release{m} which established a \CP edge from the \Release{m} by \code{T} to the
\Acquire{m} by \code{T'}. This event will verify all \PCP elements which depend
on \code{m}. \VC associates a vector clock with each thread. These vector clocks
work in the same fashion that the FastTrack algorithm tracks vector clocks per
thread. \VC also extends the lock elements discussed in
section~\ref{LockSetElements}.
\begin{itemize}
  \item \textbf{\VCHBLock{m}{v}{T()}} = if \VCHBLock{m}{v}{T()} $\in$
  \HBLockSet{x}{}, then \LastAccess{x} \HBRelation \Release{m} by \code{T}, for
  minimum version $v$ and current \VC of thread \code{T}: $T()$.
   
  \item \textbf{\VCLSLock{m}{v}{T()}} = if \VCLSLock{m}{v}{T()} $\in$
  \HBLockSet{x}{}, then \Acquire{m} by \code{T} \HBRelation \LastAccess{x}, for
  a minimum version $v$, $\wedge$ \LastAccess{x} \HBRelation
  \Release{m} by \code{T}, of the same version $v$; and current \VC of thread
  \code{T}: $T()$
\end{itemize}
These \VC elements verify if \RuleB has been established once a \CP edge gives
\CP ordering to the \Release{m}. To verify a \CP edge must first be established
within the enclosing critical section on \code{m}. Once \CP is established, the
variables that are establishing \CP on lock \code{n} will compare
\VCHBLock{m}{v}{Tx()} from \HBLockSet{x}{} to \VCHBLock{n}{w}{Ty()} from
\CPLockSet{x}{}. If $Tx = Ty$ then $v < w$ to verify \RuleB. Otherwise, if $Tx
\neq Ty$ then $v \leq Ty(Tx)$ to verify \RuleB.


==> CheckRace.tex <==
%auto-ignore
\begin{algorithm}[h] \caption{\label{CheckRace}\hfill CheckRace(\code{p})}
	\begin{algorithmic}
		\IF {$\code{p} \text{ represents variable } \code{y} \mid \RaceElement{y}{i}{T} \in \RaceSet$}
			\IF {$\CPThread{T} \in \CPLockSet{y}{i}$}
				\STATE remove \RaceElement{y}{i}{T} from \RaceSet
				\STATE $\HBLockSet{y}{i}, \CPLockSet{y}{i}, \PCPLockSet{y}{i} \leftarrow \emptyset$
			\ELSIF {$\PCPLockSet{y}{i} = \emptyset$}
				\STATE report race on \code{y}
				\STATE $\HBLockSet{y}{i}, \CPLockSet{y}{i}, \PCPLockSet{y}{i} \leftarrow \emptyset$
			\ENDIF
		\ENDIF
	\end{algorithmic} \label{alg:raceCheck}
\end{algorithm}

==> Other-Proofs.tex <==
%auto-ignore
\paragraph{Proof of \HBinv for \Acquire{m}{i}.}

Let $\rhsSet{} = \myset{\rhoprime \mid \big(\exists e' \mid \comp{\rhoprime}{e'} \land \HBOrdered{\erho}{e'} \totalOrder e\big)}$.

\mike{Missing from both directions: line~\ref{line:acq:initialize-HB}}

\begin{description}
\item[Subset direction] Let $\rhoprime \in \HBLockSetPlain{\rho}{}^+$.

If $\rhoprime \in \HBLockSetPlain{\rho}{}$,
then $\exists e' \mid \comp{\rhoprime}{e'} \land \HBOrdered{\erho}{e'} \totalOrder e$ by the inductive hypothesis.
Since $e \totalOrder e^+$ and thus $\HBOrdered{\erho}{e'} \totalOrder e^+$, $\rhoprime \in \rhsSet{+}$.

If line~\ref{line:acq:HBEdge-Established} evaluates to true for $\rho$,
then $\exists j \mid \HBLock{m}{j} \in \HBLockSetPlain{\rho}{}$,
and line~\ref{line:acq:add-HBThread} executes, so $\thr{T} \in \HBLockSetPlain{\rho}{}^+$.
By the inductive hypothesis,
$\exists j \mid \HBOrdered{\erho}{\Release{m}{j}} \totalOrder e$.
By the definition of \HB, \HBOrdered{\Release{m}{j}}{e} and thus \HBOrdered{\erho}{e}.
Since $\getThread{e} = \thr{T}$ and $\HBOrdered{\erho}{e} \totalOrder e^+$,
$\thr{T} \in \rhsSet{+}$.

\item[Superset direction] Let $\rhoprime \in \rhsSet{+}$.
Thus $\exists e' \mid \comp{\rhoprime}{e'} \land \HBOrdered{\erho}{e'} \totalOrder e^+$.

If $\rhoprime \in \HBLockSetPlain{\rho}{}$,
then $\rhoprime \in \HBLockSetPlain{\rho}{}^+$ since Algorithm~\ref{alg:acquire} maintains $\HBLockSetPlain{\rho}{}^+ \supseteq \HBLockSetPlain{\rho}{}$.

Otherwise ($\rhoprime \notin \HBLockSetPlain{\rho}{}$),
$\nexists e'' \mid \comp{\rhoprime}{e''} \land \HBOrdered{\erho}{e''} \totalOrder e$,
which implies $e' = e$.
Since $\comp{\rhoprime}{e} \land \HBOrdered{\erho}{e} \totalOrder e^+$ and $e = \Acquire{m}{i}$ by \thr{T},
$\rhoprime = \thr{T}$.
Since $\nexists e'' \mid \getThread{e''} = \thr{T} \land \HBOrdered{\erho}{e''} \totalOrder e$,
$\exists j \mid \HBOrdered{\erho}{\Release{m}{j}} \totalOrder e$
by the definition of \HB.
\mike{The above sentence is true, but it feels like a leap from the previously stated facts.}
Thus $\HBLock{m}{j} \in \HBLockSetPlain{\rho}{}$ by the inductive hypothesis.
Therefore line~\ref{line:acq:HBEdge-Established} in Algorithm~\ref{alg:acquire} evaluates to true for $\rho$,
so line~\ref{line:acq:add-HBThread} executes, adding \thr{T} to $\HBLockSetPlain{\rho}{}^+$.

\end{description}


==> PCPTrigger.tex <==
%auto-ignore
\begin{algorithm}[h] \caption{\label{TriggerPCP}\hfill TriggerPCP(\code{p}, \HBLock{m}{v})}
	\begin{algorithmic} [1]
		\State \mike{What's \code{m} here? Where does it come from?}
		\mike{In any case, I think this can be inlined into the algorithm for release, assuming we remove it from the algorithm for write.
		\jake{I agree, but I will leave it here until the comments are fully addressed for \Release{m}{v}}}
		\ForAll {$\PCPLock{n}{m}{v} \in \PCPLockSet{p}{}$}
			\State add \CPLock{n} to \CPLockSet{p}{}
% 			\mike{Incorrectly gives the impression that locks and threads are added as pairs.
% 			Use a variable that could be a lock or thread, or use separate loops.} 
			\State remove \PCPLock{n}{m}{v} from \PCPLockSet{p}{}
		\EndFor
		\ForAll {$\PCPThread{T}{m}{v} \in \PCPLockSet{p}{}$}
			\State add \CPThread{T} to \CPLockSet{p}{}
			\State remove \PCPThread{T}{m}{v} from \PCPLockSet{p}{}
		\EndFor
	\end{algorithmic}
\end{algorithm}



==> Read-Details.tex <==
%auto-ignore
\section{Detailed Analysis Changes for Reads}
\label{sec:read-details}

This section presents \raptor's analysis that handles not only writes but also reads,
corresponding to the changes described in Section~\ref{sec:reads}.
Algorithm~\ref{readEvent} adds analysis steps to handle a read event.
Algorithm~\ref{modWriteEvent} extends the analysis for a write event (Algorithm~\ref{alg:write}) to handle the existence of reads.
Algorithm~\ref{modVariableRemoval} modifies the analysis that removes obsolete variable locksets and detects \races (Algorithm~\ref{alg:varRemoval}) to handle reads.

% \mike{TODO: modify Algorithm~\ref{modVariableRemoval} to look like Algorithm~\ref{alg:varRemoval}.}

\begin{algorithm}[h] \caption{\label{readEvent}\hfill \Read{x}{i}{T} by \thr{T}}
\notes{
\mike{I think these algorithms are out of date w.r.t.\ the latest changes to the algorithms in Section~\ref{sec:analysis}.}
}
	\begin{algorithmic}[1]	
		\LineCommentx{Apply \RuleA}
		\ForAll {$\HBLock{m}{} \in \heldBy{T}$}
			\lIf{$\exists j \exists h \mid \LSLock{m}{j} \in \HBLockSet{x}{h} \land \CPThread{T} \notin \POLockSet{x}{h}$}{\Add{\CPThread{T}}{\CPLockSet{m}{j}} s.t.\ $j$ is max satisfying index}
% 			\If {$\exists j \exists h \mid \LSLock{m}{j} \in \HBLockSet{x}{h} \land \CPThread{T} \notin \POLockSet{x}{h}$}
% 			\notes{\mike{Removed $\land e_{\OwnerElement{x}{h}} = \Write{x}{h}$ since I don't think that should be there.}}
% 				\State \Add{\CPThread{T}}{\CPLockSet{m}{j}}
% 			\EndIf
		\EndFor
		\LineCommentx{Add $\xi$ to represent \thr{T} at \Read{x}{i}{T}}
		
		\lIf{$\CPThread{T} \in \POLockSet{x}{i}$}{\Add{\xi_{\code{T}}}{\POLockSet{x}{i}}}
% 		\If {$\CPThread{T} \in \POLockSet{x}{i}$}
% 			\State \Add{\xi_{\code{T}}}{\POLockSet{x}{i}}
% 		\EndIf
		\lIf{$\HBThread{T} \in \HBLockSet{x}{i}$}{\Add{\xi_{\code{T}}}{\HBLockSet{x}{i}}}
% 		\If {$\HBThread{T} \in \HBLockSet{x}{i}$}
% 			\State \Add{\xi_{\code{T}}}{\HBLockSet{x}{i}}
% 		\EndIf
		\lIf{$\CPThread{T} \in \CPLockSet{x}{i}$}{\Add{\xi_{\code{T}}}{\CPLockSet{x}{i}}}
% 		\If {$\CPThread{T} \in \CPLockSet{x}{i}$}
% 			\State \Add{\xi_{\code{T}}}{\CPLockSet{x}{i}}
% 		\EndIf
		\lForAll{$\HBLock{m}{} \mid \PCPThread{T}{m}{} \in \PCPLockSet{x}{i}$}{\Add{\PCPThreadPlain{\xi_{\code{T}}}{m}{}}{\PCPLockSet{x}{i}}}
% 		\ForAll {$\HBLock{m}{} \mid \PCPThread{T}{m}{} \in \PCPLockSet{x}{i}$}
% 			\State \Add{\PCPThreadPlain{\xi_{\code{T}}}{m}{}}{\PCPLockSet{x}{i}}
% 		\EndFor
		
		\LineComment{Reset locksets if $x^i_{\code{T}}$ already exists}
		\lIf{$\thr{T} \in \POLockSetRead{x}{i}{T}$}{$\POLockSetRead{x}{i}{\code{T}} \leftarrow \emptyset, \HBLockSetRead{x}{i}{\code{T}} \leftarrow \emptyset, \CPLockSetRead{x}{i}{\code{T}} \leftarrow \emptyset, \PCPLockSetRead{x}{i}{\code{T}} \leftarrow \emptyset$}
% 		\If {$\thr{T} \in \POLockSetRead{x}{i}{T}$}
% 			\State $\POLockSetRead{x}{i}{\code{T}} \leftarrow \emptyset, \HBLockSetRead{x}{i}{\code{T}} \leftarrow \emptyset$
% 			\State $\CPLockSetRead{x}{i}{\code{T}} \leftarrow \emptyset, \PCPLockSetRead{x}{i}{\code{T}} \leftarrow \emptyset$
% 		\EndIf
		\LineCommentx{Initialize locksets for $\OwnerElement{x}{i}_T$}
		\State $\POLockSetRead{x}{i}{\code{T}} \leftarrow \{\thr{T}\}$
		\State $\HBLockSetRead{x}{i}{\code{T}} \leftarrow \{\thr{T}\} \cup \{\LSLock{m}{j} \mid \HBLock{m}{j} \in \heldBy{T}\}$
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h] \caption{\label{modWriteEvent}\hfill \Write{x}{i} by \code{T} [modified to handle reads]}
\notes{
\mike{I think these algorithms are out of date w.r.t.\ the latest changes to the algorithms in Section~\ref{sec:analysis}.}
}
\begin{algorithmic}[1]
	    \LineComment{Apply \RuleA}
	    \ForAll {$\HBLock{m}{} \in \heldBy{T}$}
	    	\lIf{$\exists j \exists h \mid \LSLock{m}{j} \in \HBLockSet{x}{h} \land \CPThread{T} \notin \POLockSet{x}{h}$}{\Add{\CPThread{T}}{\CPLockSet{m}{j}} s.t.\ $j$ is max satisfying index}
% 	    	\If {$\exists j \exists h \mid \LSLock{m}{j} \in \HBLockSet{x}{h} \land \CPThread{T} \notin \POLockSet{x}{h}$}
% 				\State \Add{\CPThread{T}}{\CPLockSet{m}{j}}
% 			\EndIf
			\ForAll {threads \thr{t}}
				\lIf{$\exists j \exists h \mid \LSLock{m}{j} \in \HBLockSetRead{x}{h}{\code{t}} \land \CPThread{T} \notin \POLockSetRead{x}{h}{\code{t}}$}{\Add{\CPThread{T}}{\CPLockSet{m}{j}} {\smaller s.t.\ $j$ is max satisfying index}}
% 				\If {$\exists j \exists h \mid \LSLock{m}{j} \in \HBLockSetRead{x}{h}{\code{t}} \land \CPThread{T} \notin \POLockSetRead{x}{h}{\code{t}}$}
% 					\State \Add{\CPThread{T}}{\CPLockSet{m}{j}}
% 				\EndIf
			\EndFor
	    \EndFor
		\LineCommentx{Add $\xi$ to represent \thr{T} at \Write{x}{i}}
		
		\lIf{$\CPThread{T} \in \POLockSet{x}{i-1}$}{\Add{\xi}{\POLockSet{x}{i-1}}}
% 		\If {$\CPThread{T} \in \POLockSet{x}{i-1}$}
% 			\State \Add{\xi}{\POLockSet{x}{i-1}}
% 		\EndIf
		\lIf{$\HBThread{T} \in \HBLockSet{x}{i-1}$}{\Add{\xi}{\HBLockSet{x}{i-1}}}
% 		\If {$\HBThread{T} \in \HBLockSet{x}{i-1}$}
% 			\State \Add{\xi}{\HBLockSet{x}{i-1}}
% 		\EndIf
		\lIf{$\CPThread{T} \in \CPLockSet{x}{i-1}$}{\Add{\xi}{\CPLockSet{x}{i-1}}}
% 		\If {$\CPThread{T} \in \CPLockSet{x}{i-1}$}
% 			\State \Add{\xi}{\CPLockSet{x}{i-1}}
% 		\EndIf
		\lForAll{$\HBLock{m}{} \mid \PCPThread{T}{m}{} \in \PCPLockSet{x}{i-1}$}{\Add{\PCPThreadPlain{\xi}{m}{}}{\PCPLockSet{x}{i-1}}}
% 		\ForAll {$\HBLock{m}{} \mid \PCPThread{T}{m}{} \in \PCPLockSet{x}{i-1}$}
% 			\State \Add{\PCPThreadPlain{\xi}{m}{}}{\PCPLockSet{x}{i-1}}
% 		\EndFor
		
		\ForAll {threads \thr{t}}
			\lIf{$\CPThread{T} \in \POLockSetRead{x}{i-1}{\code{t}}$}{\Add{\xi}{\POLockSetRead{x}{i-1}{\code{t}}}}
% 			\If {$\CPThread{T} \in \POLockSetRead{x}{i-1}{\code{t}}$}
% 				\State \Add{\xi}{\POLockSetRead{x}{i-1}{\code{t}}}
% 			\EndIf
			\lIf{$\HBThread{T} \in \HBLockSetRead{x}{i-1}{\code{t}}$}{\Add{\xi}{\HBLockSetRead{x}{i-1}{\code{t}}}}
% 			\If {$\HBThread{T} \in \HBLockSetRead{x}{i-1}{\code{t}}$}
% 				\State \Add{\xi}{\HBLockSetRead{x}{i-1}{\code{t}}}
% 			\EndIf
			\lIf{$\CPThread{T} \in \CPLockSetRead{x}{i-1}{\code{t}}$}{\Add{\xi}{\CPLockSetRead{x}{i-1}{\code{t}}}}
% 			\If {$\CPThread{T} \in \CPLockSetRead{x}{i-1}{\code{t}}$}
% 				\State \Add{\xi}{\CPLockSetRead{x}{i-1}{\code{t}}}
% 			\EndIf
			\lForAll{$\HBLock{m}{} \mid \PCPThread{T}{m}{} \in \PCPLockSetRead{x}{i-1}{\code{t}}$}{\Add{\PCPThreadPlain{\xi}{m}{}}{\PCPLockSetRead{x}{i-1}{\code{t}}}}
% 			\ForAll {$\HBLock{m}{} \mid \PCPThread{T}{m}{} \in \PCPLockSetRead{x}{i-1}{\code{t}}$}
% 				\State \Add{\PCPThreadPlain{\xi}{m}{}}{\PCPLockSetRead{x}{i-1}{\code{t}}}
% 			\EndFor
		\EndFor
		\LineComment{Initialize locksets for \HBLock{x}{i}}
		\State $\POLockSet{x}{i} \leftarrow \{\code{T}\}$
		\State $\HBLockSet{x}{i} \leftarrow \{\HBThread{T}\} \cup \{\LSLock{m}{j} \mid \HBLock{m}{j} \in \heldBy{T}\}$ \label{wr:newLockset}
	\end{algorithmic}
% 	\label{alg:write}
\end{algorithm}

\begin{algorithm}[h] \caption{\label{modVariableRemoval}\hfill Detect and remove obsolete locksets and report \races for \OwnerElement{x}{i} and $\OwnerElement{x}{i}_\thr{t}$ (for all threads \thr{t})} \begin{algorithmic} [1]
\notes{
\mike{I think these algorithms are out of date w.r.t.\ the latest changes to the algorithms in Section~\ref{sec:analysis}.}
}
		\If {$\Write{x}{i+1}$ has executed}
			\lIf {$\xi \notin \CPLockSet{x}{i} \cup \POLockSet{x}{i} \land \nexists \HBLock{m}{j} \mid \PCPThreadPlain{\xi}{m}{j} \in \PCPLockSet{x}{i}$}{Report \race between \Write{x}{i} and \Write{x}{i+1}}
	 		\ForAll{threads \thr{t}}
	 			\lIf {$\xi_t \notin \CPLockSet{x}{i} \cup \POLockSet{x}{i} \land \nexists \HBLock{m}{j} \mid \PCPThreadPlain{\xi_t}{m}{j} \in \PCPLockSet{x}{i}$}{Report \race between \Write{x}{i} and \Read{x}{i}{t}}
	 			\If{$\xi \in \CPLockSetRead{x}{i}{t} \cup \POLockSetRead{x}{i}{t}$}
	 				\State $\POLockSetRead{x}{i}{t}^+ \leftarrow \emptyset\,$, $\HBLockSetRead{x}{i}{t}^+ \leftarrow \emptyset\,$, $\CPLockSetRead{x}{i}{t}^+ \leftarrow \emptyset\,$, $\PCPLockSetRead{x}{i}{t}^+ \leftarrow \emptyset$
					{\smaller \Comment{No read--write \race}}
				\ElsIf{$\nexists \HBLock{m}{j} \mid \PCPThreadPlain{\xi}{m}{j} \in \PCPLockSetRead{x}{i}{t}$}{ Report \race between \Read{x}{i}{t} and \Write{x}{i+1}}
				\EndIf
	 		\EndFor
	 		\If {$\nexists \HBLock{m}{j} \mid \PCPThreadPlain{\xi}{m}{j} \in \PCPLockSet{x}{i} \land \forall \text{threads \thr{t} } \nexists \HBLock{m}{j} \mid \PCPThreadPlain{\xi_\thr{t}}{m}{j} \in \PCPLockSet{x}{i}$}
				\State $\POLockSet{x}{i}^+ \leftarrow \emptyset\,$, $\HBLockSet{x}{i}^+ \leftarrow \emptyset\,$, $\CPLockSet{x}{i}^+ \leftarrow \emptyset\,$, $\PCPLockSet{x}{i}^+ \leftarrow \emptyset$
	 			{\smaller \Comment{No \race (unless reported above)}}
	 		\EndIf
		\EndIf
	\end{algorithmic}
\end{algorithm}

==> Theorems.tex <==
%auto-ignore
\section{Correctness}


==> examples/LessSimpleExample_RelationAndState.tex <==
\begin{figure}[t]
\vspace*{-1em}
\small
\centering
\begin{tabular}{lll}
Thread 1 & Thread 2 & Updated analysis state after event\\\hline
\Write{x}{1} & & $\POOrdered{\Write{x}{1}}{\Write{x}{1}}
\rightarrow \POLockSet{x}{1} = \{\HBThread{T1}\}$\\
& & $\HBOrdered{\Write{x}{1}}{\Write{x}{1}}
\rightarrow \HBLockSet{x}{1} = \{\HBThread{T1}\}$\\
\Acquire{m}{1} & & \\
\Write{y}{1} & & \\
\Release{m}{1}\tikzmark{1}{} & & $\HBOrdered{\Write{x}{1}}{\Release{m}{1}}
\rightarrow \HBLockSet{x}{1} = \{\HBThread{T1}, \HBLock{m}{1}\}$\\
& \tikzmark{2}{}\Acquire{m}{2} & $\HBOrdered{\Write{x}{1}}{\Acquire{m}{2}} 
\rightarrow \HBLockSet{x}{1} = \{\HBThread{T1}, \HBThread{T2}, \HBLock{m}{1}\}$,
$\PCPOrdered{\Write{x}{1}}{\Acquire{m}{2}}
\rightarrow \PCPLockSet{x}{1} = \{\PCPThread{T2}{m}{1}\}$\\
& \Write{x}{2} & $\PCPOrdered{\Write{x}{1}}{\Write{x}{2}}
\rightarrow \PCPLockSet{x}{1} = \{\PCPThread{T2}{m}{1}, \PCPThreadPlain{\xi}{m}{1}\}$\\
& \textbf{\Write{y}{2}} & $\CPOrdered{\Release{m}{1}}{\Acquire{m}{2}}
\rightarrow \CPLockSet{m}{1} = \{\CPThread{T2}\}$\\
& \Release{m}{2} & $\CPOrdered{\Write{x}{1}}{\Acquire{m}{2}} 
\rightarrow \CPLockSet{x}{1} = \{\CPThread{T2}, \CPLock{m}\}$,
$\CPOrdered{\Write{x}{1}}{\Write{x}{2}}
\rightarrow \CPLockSet{x}{1} = \{\CPThread{T2}, \CPLock{m}, \CPThreadPlain{\xi}\}$\\
& & $\CPOrdered{\Acquire{m}{1}}{\Release{m}{2}}
\rightarrow \CPLockSet{m}{1} = \{\CPThread{T2}, \CPLock{m}\}$\\
\end{tabular}
\link{1}{2}

\mike{The last column seems confusing. I think it needs to show \emph{all} updated state, like Figure~\ref{fig:simple-analysis-example}.
It could also include some explanations for some updates, but I think the explanations that are there now are confusing.}

\mike{In any case, I don't think we should show this example in the paper.
I think we should show two examples with analysis state updates:
the example from Figure~\ref{fig:SimpleExample:no-CP-race} and the example from Figure~\ref{fig:LessComplexExample}.
We can also keep Figure~\ref{}, but we may want to move it to supplementary material.}

\caption{\label{fig:SimpleExample:raptor-state} An executions in which \code{x}
and \code{y} are shared variables, and \code{m} is a lock.
In this execution, the state Raptor tracks is represented as locksets
corresponding to the relations established.}
\end{figure}

==> examples/RuleBLateVariableAccess.tex <==
\begin{figure}
\smaller
\centering

\newcolumntype{L}{>{$}l<{$}} % math-mode version of "l" column type

\begin{tabular}{@{}l@{\;}l@{\;\;}l@{\;}l@{\;}|L@{}}
\thr{T1} & \thr{T2} & \thr{T3} & \thr{T4} & \text{Updated analysis state after event (excluding \POLockSetPlain{\rho}{})}\\\hline
&\Acquire{m}{1}&&& \HBLockSet{m}{1} = \{\HBThread{T2}\}\\
&\Acquire{q}{1}&&& \HBLockSet{q}{1} = \{\HBThread{T2}\}\\
&\Release{q}{1}&&& \HBLockSet{m}{1} = \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBThread{T2}\}\\
&&\Acquire{q}{2}&& \HBLockSet{q}{2} = \{\HBThread{T3}\}, \HBLockSet{m}{1} = \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBThread{T2}, \HBThread{T3}\}, \PCPLockSet{m}{1} = \PCPLockSet{q}{1} = \{\PCPThread{T3}{q}{1}\}\\
&&\Release{q}{2}&& \HBLockSet{q}{2} = \{\HBLock{q}{2}, \HBThread{T3}\}, \CCPLockSet{m}{1} = \CCPLockSet{q}{1} = \emptyset\\
&&\Acquire{n}{1}&& \HBLockSet{n}{1} = \{\HBThread{T3}\}\\
&&\Write{y}{1}&& \HBLockSet{y}{1} = \{\LSLock{n}{1}, \HBThread{T3}\}\\
&&\Release{n}{1}\tikzmark{1}&& \HBLockSet{q}{2} = \{\HBLock{q}{2}, \HBLock{n}{1}, \HBThread{T3}\}, \HBLockSet{n}{1} = \{\HBLock{n}{1}, \HBThread{T3}\}, \HBLockSet{m}{1} = \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBLock{n}{1}, \HBThread{T2}, \HBThread{T3}\}\\
&&&\tikzmark{2}\Acquire{n}{2}& \HBLockSet{y}{1} = \{\LSLock{n}{1}, \HBThread{T3}, \HBThread{T4}\}, \HBLockSet{q}{2} = \{\HBLock{q}{2}, \HBLock{n}{1}, \HBThread{T3}, \HBThread{T4}\}, \HBLockSet{n}{1} = \{\HBLock{n}{1}, \HBThread{T3}, \HBThread{T4}\},\\
&&&& \HBLockSet{m}{1} = \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBLock{n}{1}, \HBThread{T2}, \HBThread{T3}, \HBThread{T4}\}, \HBLockSet{n}{2} = \{\HBThread{T4}\},\\
&&&& \PCPLockSet{m}{1} = \PCPLockSet{q}{1} = \PCPLockSet{q}{2} = \PCPLockSet{n}{1} = \PCPLockSet{y}{1} = \{\PCPThread{T4}{n}{1}\}\\
&&&\Write{y}{2}& \HBLockSet{y}{1} = \{\LSLock{n}{1}, \HBThread{T3}, \HBThread{T4}, \HBThreadPlain{\xi}\}, \HBLockSet{y}{2} = \{\LSLock{n}{2}, \HBThread{T4}\}, \CPLockSet{n}{1} = \{\CPThread{T4}\}, \PCPLockSet{y}{1} = \{\PCPThread{T4}{n}{1}, \PCPThread{$\xi$}{n}{1}\}\\
&&&\Release{n}{2}& \HBLockSet{n}{2} = \{\HBLock{n}{2}, \HBThread{T4}\}, \CPLockSet{y}{1} = \{\CPLock{n}, \CPThread{T4}, \CPThread{$\xi$}\}, \CPLockSet{m}{1} = \CPLockSet{q}{1} = \CPLockSet{q}{2} = \CPLockSet{n}{1} = \{\CPLock{n}, \CPThread{T4}\},\\
&&&& \PCPLockSet{m}{1} = \PCPLockSet{q}{1} = \PCPLockSet{q}{2} = \PCPLockSet{n}{1} = \PCPLockSet{y}{1} = \emptyset\\
\Write{x}{1}&&&& \HBLockSet{x}{1} = \{\HBThread{T1}\}\\
\Acquire{p}{1}&&&& \HBLockSet{p}{1} = \{\HBThread{T1}\}\\
\Release{p}{1}&&&& \HBLockSet{p}{1} = \HBLockSet{x}{1} = \{\HBLock{p}{1}, \HBThread{T1}\},\\
&\Acquire{p}{2}&&& \HBLockSet{p}{1} = \HBLockSet{x}{1} = \{\HBLock{p}{1}, \HBThread{T1}, \HBThread{T2}\}, \HBLockSet{p}{2} = \{\HBThread{T2}\}, \PCPLockSet{p}{1} = \PCPLockSet{x}{1} = \{\PCPThread{T2}{p}{1}\}\\
&\Release{p}{2}&&& \HBLockSet{m}{1} = \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBLock{n}{1}, \HBLock{p}{2}, \HBThread{T2}, \HBThread{T3}, \HBThread{T4}\}, \HBLockSet{p}{2} = \{\HBLock{p}{2}, \HBThread{T2}\},\\
&&&& \CCPLockSet{p}{1} = \CCPLockSet{x}{1} = \emptyset\\
&\Release{m}{1}&&& \HBLockSet{p}{1} = \HBLockSet{x}{1} = \{\HBLock{p}{1}, \HBLock{m}{1}, \HBThread{T1}, \HBThread{T2}\}, \HBLockSet{m}{1} = \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBLock{n}{1}, \HBLock{p}{2}, \HBLock{m}{1}, \HBThread{T2}, \HBThread{T3}, \HBThread{T4}\}\\
&&&& \HBLockSet{p}{2} = \{\HBLock{p}{2}, \HBLock{m}{1}, \HBThread{T2}\}\\
&&&\Acquire{m}{2}& \HBLockSet{p}{1} = \HBLockSet{x}{1} = \{\HBLock{p}{1}, \HBLock{m}{1}, \HBThread{T1}, \HBThread{T2}, \HBThread{T4}\}, \HBLockSet{p}{2} = \{\HBLock{p}{2}, \HBLock{m}{1}, \HBThread{T2}, \HBThread{T4}\}, \HBLockSet{m}{2} = \{\HBThread{T4}\}\\
&&&& \PCPLockSet{p}{1} = \PCPLockSet{p}{2} = \PCPLockSet{x}{1} = \PCPLockSet{m}{1} = \PCPLockSet{q}{1} = \{\PCPThread{T4}{m}{1}\}\\
&&&\Release{m}{2}& \HBLockSet{m}{2} = \{\HBLock{m}{2}, \HBThread{T4}\}, \HBLockSet{n}{2} = \{\HBLock{n}{2}, \HBLock{m}{2}, \HBThread{T4}\}, \HBLockSet{y}{1} = \{\LSLock{n}{1}, \HBLock{m}{2}, \HBThread{T3}, \HBThread{T4}, \HBThreadPlain{\xi}\},\\
&&&& \HBLockSet{q}{2} = \{\HBLock{q}{2}, \HBLock{n}{1}, \HBLock{m}{2}, \HBThread{T3}, \HBThread{T4}\}, \HBLockSet{y}{2} = \{\LSLock{n}{2}, \HBLock{m}{2}, \HBThread{T4}\}, \HBLockSet{n}{1} = \{\HBLock{n}{1}, \HBLock{m}{2}, \HBThread{T3}, \HBThread{T4}\},\\
&&&& \CPLockSet{p}{1} = \CPLockSet{p}{2} = \CPLockSet{x}{1} = \{\CPLock{m}, \CPThread{T4}\}, \CPLockSet{y}{1} = \{\CPLock{n}, \CPLock{m}, \CPThread{T4}, \CPThread{$\xi$}\},\\
&&&& \CPLockSet{m}{1} = \CPLockSet{q}{1} = \CPLockSet{q}{2} = \CPLockSet{n}{1} = \{\CPLock{n}, \CPLock{m}, \CPThread{T4}\},\\
&&&& \CCPLockSet{p}{1} = \CCPLockSet{p}{2} = \CCPLockSet{x}{1} = \CCPLockSet{m}{1} = \CCPLockSet{q}{1} = \emptyset\\
&&&\Write{x}{2}& \HBLockSet{x}{2} = \{\HBThread{T4}\}, \CPLockSet{x}{1} = \{\CPLock{m}, \CPThread{T4}, \CPThreadPlain{\xi}\}, \HBLockSet{x}{1} = \{\HBLock{p}{1}, \HBLock{m}{1}, \HBThread{T1}, \HBThread{T2}, \HBThread{T4}, \HBThreadPlain{\xi} \}\\

\end{tabular}
\textlink{1}{2}{\CP}

% \mike{Shouldn't \CPLockSet{x}{1} and \HBLockSet{x}{1} contain $\xi$ after \Write{x}{2}?
% \mike{Jake!}}

% \mike{I think all examples should use \thr{T1} etc.\ (since those are in fact lockset elements used by the analysis). I'll make this change.}

\caption{Example execution and \goldCP's analysis state.
\CPOrdered{\Write{x}{1}}{\Write{x}{2}} because \CPOrdered{\Release{n}{1}}{\Acquire{n}{2}}, yet
\Write{x}{1} executes only after \CPOrdered{\Release{n}{1}}{\Acquire{n}{2}} has been established
and after \Release{n}{2} has executed.}
\label{fig:ruleb-late-variable-access}
\end{figure}

==> examples/TrickyFalseRuleB.tex <==
\begin{figure}
\smaller
\centering

\newcolumntype{L}{>{$}l<{$}} % math-mode version of "l" column type

\begin{tabular}{@{}l@{\;}l@{\;\;}l@{\;}l@{\;}|L@{}}
\thr{T1} & \thr{T2} & \thr{T3} & \thr{T4} & \text{Updated analysis state after event (excluding \POLockSetPlain{\rho}{})}\\\hline
\Write{z}{1}&&&& \HBLockSet{z}{1} = \{\HBThread{T1}\}\\
\Acquire{q}{1}&&&& \HBLockSet{q}{1} = \{\HBThread{T1}\}\\
\Release{q}{1}&&&& \HBLockSet{z}{1} = \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBThread{T1}\}\\
\Acquire{m}{1}&&&& \HBLockSet{m}{1} = \{\HBThread{T1}\}\\
\Release{m}{1}&&&& \HBLockSet{m}{1} = \{\HBLock{m}{1}, \HBThread{T1}\}, \HBLockSet{z}{1} = \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBLock{m}{1}, \HBThread{T1}\}\\
&\Acquire{q}{2}&&& \HBLockSet{q}{2} = \{\HBThread{T2}\}, \HBLockSet{z}{1} = \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBLock{m}{1}, \HBThread{T1}, \HBThread{T2}\}, \PCPLockSet{z}{1} = \PCPLockSet{q}{1} = \{\PCPThread{T2}{q}{1}\}\\
&\Release{q}{2}&&& \HBLockSet{q}{2} = \{\HBLock{q}{2}, \HBThread{T2}\}, \CCPLockSet{z}{1} = \CCPLockSet{q}{1} = \emptyset\\
&\Acquire{n}{1}&&& \HBLockSet{n}{1} = \{\HBThread{T2}\}\\
&\Write{y}{1}&&& \HBLockSet{y}{1} = \{\LSLock{n}{1}, \HBThread{T2}\}\\
&\Release{n}{1}\tikzmark{1}&&& \HBLockSet{n}{1} = \{\HBLock{n}{1}, \HBThread{T2}\}, \HBLockSet{q}{2} = \{\HBLock{q}{2}, \HBLock{n}{1}, \HBThread{T2}\}, \HBLockSet{z}{1} = \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBLock{m}{1}, \HBLock{n}{1}, \HBThread{T1}, \HBThread{T2}\}\\
&&\Acquire{m}{2}&& \HBLockSet{z}{1} = \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBLock{m}{1}, \HBLock{n}{1}, \HBThread{T1}, \HBThread{T2}, \HBThread{T3}\}, \HBLockSet{m}{1} = \{\HBLock{m}{1}, \HBThread{T1}, \HBThread{T3}\}, \HBLockSet{m}{2} = \{\HBThread{T3}\},\\
&&&& \PCPLockSet{z}{1} = \PCPLockSet{q}{1} = \PCPLockSet{m}{1} = \{\PCPThread{T3}{m}{1}\}\\
&&\Acquire{o}{1}&& \HBLockSet{o}{1} = \{\HBThread{T3}\}\\
&&\Release{o}{1}&& \HBLockSet{z}{1} = \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBLock{m}{1}, \HBLock{n}{1}, \HBLock{o}{1}, \HBThread{T1}, \HBThread{T2}, \HBThread{T3}\}, \HBLockSet{m}{1} = \{\HBLock{m}{1}, \HBLock{o}{1}, \HBThread{T1}, \HBThread{T3}\},\\
&&&& \HBLockSet{o}{1} = \HBLockSet{m}{2} = \{\HBLock{o}{1}, \HBThread{T3}\}, \PCPLockSet{z}{1} = \PCPLockSet{q}{1} = \PCPLockSet{m}{1} = \{\PCPLock{o}{m}{1}, \PCPThread{T3}{m}{1}\}\\
&&&\Acquire{o}{2}& \HBLockSet{z}{1} = \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBLock{m}{1}, \HBLock{n}{1}, \HBLock{o}{1}, \HBThread{T1}, \HBThread{T2}, \HBThread{T3}, \HBThread{T4}\}, \HBLockSet{m}{1} = \{\HBLock{m}{1}, \HBLock{o}{1}, \HBThread{T1}, \HBThread{T3}, \HBThread{T4}\},\\
&&&& \HBLockSet{o}{1} = \HBLockSet{m}{2} = \{\HBLock{o}{1}, \HBThread{T3}, \HBThread{T4}\}, \HBLockSet{o}{2} = \{\HBThread{T4}\}, \PCPLockSet{o}{1} = \PCPLockSet{m}{2} = \{\PCPThread{T4}{o}{1}\},\\
&&&& \PCPLockSet{z}{1} = \PCPLockSet{q}{1} = \PCPLockSet{m}{1} = \{\PCPLock{o}{m}{1}, \PCPThread{T3}{m}{1}, \PCPThread{T4}{m}{1}, \PCPThread{T4}{o}{1}\}\\ 
&&&\Release{o}{2}& \HBLockSet{o}{2} = \{\HBLock{o}{2}, \HBThread{T4}\}, \PCPLockSet{z}{1} = \PCPLockSet{q}{1} = \PCPLockSet{m}{1} = \{\PCPLock{o}{m}{1}, \PCPThread{T3}{m}{1}, \PCPThread{T4}{m}{1}\},\\
&&&& \CCPLockSet{o}{1} = \CCPLockSet{m}{2} = \emptyset\\
&&&\Write{z}{2}& \HBLockSet{z}{1} = \{\HBLock{q}{1}, \HBLock{m}{1}, \HBLock{n}{1}, \HBLock{o}{1}, \HBThread{T1}, \HBThread{T2}, \HBThread{T3}, \HBThread{T4}, \HBThreadPlain{\xi}\}, \HBLockSet{z}{2} = \{\HBThread{T4}\},\\
&&&& \PCPLockSet{z}{1} = \{\PCPLock{o}{m}{1}, \PCPThread{T3}{m}{1}, \PCPThread{T4}{m}{1}, \PCPThread{$\xi$}{m}{1}\}\\
&&\tikzmark{2}\Acquire{n}{2}&& \HBLockSet{y}{1} = \{\LSLock{n}{1}, \HBThread{T2}, \HBThread{T3}\}, \HBLockSet{n}{2} = \{\HBThread{T3}\}, \HBLockSet{n}{1} = \{\HBLock{n}{1}, \HBThread{T2}, \HBThread{T3}\}, \HBLockSet{q}{2} = \{\HBLock{q}{2}, \HBLock{n}{1}, \HBThread{T2}, \HBThread{T3}\}\\
&&&& \PCPLockSet{q}{2} = \PCPLockSet{y}{1} = \PCPLockSet{n}{1} = \{\PCPThread{T3}{n}{1}\}, \PCPLockSet{q}{1} = \{\PCPLock{o}{m}{1}, \PCPThread{T3}{m}{1}, \PCPThread{T4}{m}{1}, \PCPThread{T3}{n}{1}\},\\
&&&& \PCPLockSet{z}{1} = \{\PCPLock{o}{m}{1}, \PCPThread{T3}{m}{1}, \PCPThread{T4}{m}{1}, \PCPThread{$\xi$}{m}{1}, \PCPThread{T3}{n}{1}\}\\
&&\Write{y}{2}&& \HBLockSet{y}{1} = \{\LSLock{n}{1}, \HBThread{T2}, \HBThread{T3}, \HBThreadPlain{\xi}\}, \HBLockSet{y}{2} = \{\LSLock{m}{2}, \LSLock{n}{2}, \HBThread{T3}\}, \CPLockSet{n}{1} = \{\CPThread{T3}\}, \PCPLockSet{y}{1} = \{\PCPThread{T3}{n}{1}, \PCPThread{$\xi$}{n}{1}\}\\
&&\Release{n}{2}&& \HBLockSet{m}{1} = \{\HBLock{m}{1}, \HBLock{o}{1}, \HBLock{n}{2}, \HBThread{T1}, \HBThread{T3}, \HBThread{T4}\}, \HBLockSet{o}{1} = \HBLockSet{m}{2} = \{\HBLock{o}{1}, \HBLock{n}{2}, \HBThread{T3}, \HBThread{T4}\}, \HBLockSet{n}{2} = \{\HBLock{n}{2}, \HBThread{T3}\}\\ 
&&&& \PCPLockSet{z}{1} = \{\PCPLock{o}{m}{1}, \CCPLock{n}{m}{1}, \PCPThread{T3}{m}{1}, \PCPThread{T4}{m}{1}, \PCPThread{$\xi$}{m}{1}\}, \CCPLockSet{q}{2} = \CCPLockSet{y}{1} = \CCPLockSet{n}{1} = \emptyset,\\
&&&& \PCPLockSet{q}{1} = \CCPLockSet{m}{1} = \{\PCPLock{o}{m}{1}, \CCPLock{n}{m}{1}, \PCPThread{T3}{m}{1}, \PCPThread{T4}{m}{1}\},\\
&&&& \CPLockSet{z}{1} = \CPLockSet{q}{1} = \CPLockSet{q}{2} = \CPLockSet{n}{1} = \{\CPLock{n}, \CPThread{T3}\}, \CPLockSet{y}{1} = \{\CPLock{n}, \CPThread{T3}, \CPThread{$\xi$}\}\\
&&\Release{m}{2}&& \HBLockSet{n}{2} = \{\HBLock{n}{2}, \HBLock{m}{2}, \HBThread{T3}\}, \HBLockSet{o}{1} = \HBLockSet{m}{2} = \{\HBLock{o}{1}, \HBLock{n}{2}, \HBLock{m}{2}, \HBThread{T3}, \HBThread{T4}\},\\
&&&& \HBLockSet{q}{2} = \{\HBLock{q}{2}, \HBLock{m}{2}, \HBLock{n}{1}, \HBThread{T2}, \HBThread{T3}\}, \HBLockSet{n}{1} = \{\HBLock{n}{1}, \HBLock{m}{2}, \HBThread{T2}, \HBThread{T3}\}, \HBLockSet{y}{1} = \{\LSLock{n}{1}, \HBLock{m}{2}, \HBThread{T2}, \HBThread{T3}, \HBThreadPlain{\xi}\},\\
&&&& \CPLockSet{z}{1} = \CPLockSet{q}{1} = \CPLockSet{q}{2} = \CPLockSet{n}{1} = \{\CPLock{n}, \CPLock{m}, \CPThread{T3}\}, \CPLockSet{y}{1} = \{\CPLock{n}, \CPLock{m}, \CPThread{T3}, \CPThread{$\xi$}\},\\
&&&& \CCPLockSet{z}{1} = \CCPLockSet{q}{1} = \emptyset

\end{tabular}
\textlink{1}{2}{\CP}
\caption{Example execution and \goldCP's analysis state.
This example is subtlely different from the example in Figure~\ref{fig:tricky-true-ruleb}:
it flips the order of \thr{T1}'s critical sections on \code{m} and \code{q}.
As a result, \protect\NotCPOrdered{\Acquire{m}{1}}{\Release{m}{2}} and \protect\NotCPOrdered{\Write{z}{1}}{\Write{z}{2}}.}
\label{fig:tricky-false-ruleb}
\end{figure}

==> examples/TrickyTrueRuleB.tex <==
\begin{figure}
\smaller
\centering

\newcolumntype{L}{>{$}l<{$}} % math-mode version of "l" column type

\begin{tabular}{@{}l@{\;}l@{\;\;}l@{\;}l@{\;}|L@{}}
\thr{T1} & \thr{T2} & \thr{T3} & \thr{T4} & \text{Updated analysis state after event (excluding \POLockSetPlain{\rho}{})}\\\hline
\Write{z}{1}&&&& \HBLockSet{z}{1} = \{\HBThread{T1}\}\\
\Acquire{m}{1}&&&& \HBLockSet{m}{1} = \{\HBThread{T1}\}\\
\Release{m}{1}&&&& \HBLockSet{z}{1} = \HBLockSet{m}{1} = \{\HBLock{m}{1}, \HBThread{T1}\}\\
\Acquire{q}{1}&&&& \HBLockSet{q}{1} = \{\HBThread{T1}\}\\
\Release{q}{1}&&&& \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBThread{T1}\}, \HBLockSet{z}{1} = \HBLockSet{m}{1} = \{\HBLock{m}{1}, \HBLock{q}{1}, \HBThread{T1}\}\\
&\Acquire{q}{2}&&& \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBThread{T1}, \HBThread{T2}\}, \HBLockSet{z}{1} = \HBLockSet{m}{1} = \{\HBLock{m}{1}, \HBLock{q}{1}, \HBThread{T1}, \HBThread{T2}\}, \HBLockSet{q}{2} = \{\HBThread{T2}\}\\
&&&& \PCPLockSet{q}{1} = \PCPLockSet{z}{1} = \PCPLockSet{m}{1} = \{\PCPThread{T2}{q}{1}\}\\
&\Release{q}{2}&&& \HBLockSet{q}{2} = \{\HBLock{q}{2}, \HBThread{T2}\}, \PCPLockSet{q}{1} = \PCPLockSet{z}{1} = \PCPLockSet{m}{1} = \emptyset\\
&\Acquire{n}{1}&&& \HBLockSet{n}{1} = \{\HBThread{T2}\}\\
&\Write{y}{1}&&& \HBLockSet{y}{1} = \{\LSLock{n}{1}, \HBThread{T2}\}\\
&\Release{n}{1}\tikzmark{1}&&& \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBLock{n}{1}, \HBThread{T1}, \HBThread{T2}\}, \HBLockSet{z}{1} = \HBLockSet{m}{1} = \{\HBLock{m}{1}, \HBLock{q}{1}, \HBLock{n}{1}, \HBThread{T1}, \HBThread{T2}\},\\ 
&&&& \HBLockSet{q}{2} = \{\HBLock{q}{2}, \HBLock{n}{1}, \HBThread{T2}\}, \HBLockSet{n}{1} = \{\HBLock{n}{1}, \HBThread{T2}\}\\
&&\Acquire{m}{2}&& \HBLockSet{z}{1} = \HBLockSet{m}{1} = \{\HBLock{m}{1}, \HBLock{q}{1}, \HBLock{n}{1}, \HBThread{T1}, \HBThread{T2}, \HBThread{T3}\}, \HBLockSet{m}{2} = \{\HBThread{T3}\}, \PCPLockSet{z}{1} = \PCPLockSet{m}{1} = \{\PCPThread{T3}{m}{1}\}\\
&&\Acquire{o}{1}&& \HBLockSet{o}{1} = \{\HBThread{T3}\}\\
&&\Release{o}{1}&& \HBLockSet{z}{1} = \HBLockSet{m}{1} = \{\HBLock{m}{1}, \HBLock{q}{1}, \HBLock{n}{1}, \HBLock{o}{1}, \HBThread{T1}, \HBThread{T2}, \HBThread{T3}\}, \HBLockSet{o}{1} = \HBLockSet{m}{2} = \{\HBLock{o}{1}, \HBThread{T3}\}\\
&&&& \PCPLockSet{z}{1} = \PCPLockSet{m}{1} = \{\PCPLock{o}{m}{1}, \PCPThread{T3}{m}{1}\}\\
&&&\Acquire{o}{2}& \HBLockSet{z}{1} = \HBLockSet{m}{1} = \{\HBLock{m}{1}, \HBLock{q}{1}, \HBLock{n}{1}, \HBLock{o}{1}, \HBThread{T1}, \HBThread{T2}, \HBThread{T3}, \HBThread{T4}\}, \HBLockSet{o}{1} = \HBLockSet{m}{2} = \{\HBLock{o}{1}, \HBThread{T3}, \HBThread{T4}\},\\
&&&& \HBLockSet{o}{2} = \{\HBThread{T4}\}, \PCPLockSet{z}{1} = \PCPLockSet{m}{1} = \{\PCPLock{o}{m}{1}, \PCPThread{T4}{m}{1}, \PCPThread{T3}{m}{1}, \PCPThread{T4}{o}{1}\}\\
&&&& \PCPLockSet{o}{1} = \PCPLockSet{m}{1} = \{\PCPThread{T4}{o}{1}\}\\
&&&\Release{o}{2}& \HBLockSet{o}{2} = \{\HBLock{o}{2}, \HBThread{T4}\}, \PCPLockSet{z}{1} = \PCPLockSet{m}{1} = \{\PCPLock{o}{m}{1}, \PCPThread{T4}{m}{1}, \PCPThread{T3}{m}{1}\}, \CCPLockSet{o}{1} = \CCPLockSet{m}{1} = \emptyset\\
&&&\Write{z}{2}& \HBLockSet{z}{2} = \{\HBThread{T4}\}, \HBLockSet{z}{1} = \{\HBLock{m}{1}, \HBLock{q}{1}, \HBLock{n}{1}, \HBLock{o}{1}, \HBThread{T1}, \HBThread{T2}, \HBThread{T3}, \HBThread{T4}, \HBThreadPlain{\xi}\},\\
&&&& \PCPLockSet{z}{1} = \{\PCPLock{o}{m}{1}, \PCPThread{T4}{m}{1}, \PCPThread{T3}{m}{1}, \PCPThread{$\xi$}{m}{1}\}\\
&&\tikzmark{2}\Acquire{n}{2}&& \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBLock{n}{1}, \HBThread{T1}, \HBThread{T2}, \HBThread{T3}\}, \HBLockSet{q}{2} = \{\HBLock{q}{2}, \HBLock{n}{1}, \HBThread{T2}, \HBThread{T3}\}, \HBLockSet{n}{1} = \{\HBLock{n}{1}, \HBThread{T2}, \HBThread{T3}\},\\
&&&& \HBLockSet{n}{2} = \{\HBThread{T3}\}, \HBLockSet{y}{1} = \{\LSLock{n}{1}, \HBThread{T2}, \HBThread{T3}\}, \PCPLockSet{m}{1} = \{\PCPLock{o}{m}{1}, \PCPThread{T4}{m}{1}, \PCPThread{T3}{m}{1}, \PCPThread{T3}{n}{1}\},\\
&&&& \PCPLockSet{z}{1} = \{\PCPLock{o}{m}{1}, \PCPThread{T4}{m}{1}, \PCPThread{T3}{m}{1}, \PCPThread{$\xi$}{m}{1}, \PCPThread{T3}{n}{1}\},\\
&&&& \PCPLockSet{y}{1} = \PCPLockSet{n}{1} = \PCPLockSet{q}{1} = \PCPLockSet{q}{2} = \{\PCPThread{T3}{n}{1}\}\\
&&\Write{y}{2}&& \HBLockSet{y}{1} = \{\LSLock{n}{1}, \HBThread{T2}, \HBThread{T3}, \HBThreadPlain{\xi}\}, \HBLockSet{y}{2} = \{\LSLock{m}{2}, \LSLock{n}{2}, \HBThread{T3}\}, \CPLockSet{n}{1} = \{\CPThread{T3}\}, \PCPLockSet{y}{1} = \{\PCPThread{T3}{n}{1}, \PCPThreadPlain{\xi}{n}{1}\}\\
&&\Release{n}{2}&& \HBLockSet{o}{1} = \HBLockSet{m}{2} = \{\HBLock{o}{1}, \HBLock{n}{2}, \HBThread{T3}, \HBThread{T4}\}, \HBLockSet{n}{2} = \{\HBLock{n}{2}, \HBThread{T3}\},\\
&&&& \CPLockSet{z}{1} = \CPLockSet{m}{1} = \CPLockSet{n}{1} = \CPLockSet{q}{1} = \CPLockSet{q}{2} = \{\CPLock{n}, \CPThread{T3}\}, \CPLockSet{y}{1} = \{\CPLock{n}, \CPThread{T3}, \CPThread{$\xi$}\},\\
&&&& \PCPLockSet{m}{1} = \{\PCPLock{o}{m}{1}, \CCPLock{n}{m}{1}, \PCPThread{T4}{m}{1}, \PCPThread{T3}{m}{1}\}, \CCPLockSet{y}{1} = \CCPLockSet{n}{1} = \CCPLockSet{q}{1} = \CCPLockSet{q}{2} = \emptyset,\\
&&&& \PCPLockSet{z}{1} = \{\PCPLock{o}{m}{1}, \CCPLock{n}{m}{1}, \PCPThread{T4}{m}{1}, \PCPThread{T3}{m}{1}, \PCPThread{$\xi$}{m}{1}\},\\
&&\Release{m}{2}&& \HBLockSet{o}{1} = \HBLockSet{m}{2} = \{\HBLock{o}{1}, \HBLock{n}{2}, \HBLock{m}{2}, \HBThread{T3}, \HBThread{T4}\}, \HBLockSet{n}{2} = \{\HBLock{n}{2}, \HBLock{m}{2}, \HBThread{T3}\}, \HBLockSet{y}{1} = \{\LSLock{n}{1}, \HBLock{m}{2}, \HBThread{T2}, \HBThread{T3}, \HBThreadPlain{\xi}\},\\
&&&& \HBLockSet{q}{1} = \{\HBLock{q}{1}, \HBLock{n}{1}, \HBLock{m}{2}, \HBThread{T1}, \HBThread{T2}, \HBThread{T3}\}, \HBLockSet{q}{2} = \{\HBLock{q}{2}, \HBLock{n}{1}, \HBLock{m}{2}, \HBThread{T2}, \HBThread{T3}\}, \HBLockSet{n}{1} = \{\HBLock{n}{1}, \HBLock{m}{2}, \HBThread{T2}, \HBThread{T3}\},\\
&&&& \CPLockSet{n}{1} = \CPLockSet{q}{1} = \CPLockSet{q}{2} = \{\CPLock{n}, \CPLock{m}, \CPThread{T3}\}, \CPLockSet{y}{1} = \{\CPLock{n}, \CPLock{m}, \CPThread{T3}, \CPThread{$\xi$}\},\\
&&&& \CPLockSet{m}{1} = \{\CPLock{n}, \CPLock{o}, \CPLock{m}, \CPThread{T3}, \CPThread{T4}\}, \CPLockSet{z}{1} = \{\CPLock{n}, \CPLock{o}, \CPLock{m}, \CPThread{T3}, \CPThread{T4}, \CPThread{$\xi$}\}, \CCPLockSet{z}{1} = \CCPLockSet{m}{1} = \emptyset

\end{tabular}
\textlink{1}{2}{\CP}
\caption{Example execution and \goldCP's analysis state.
In this execution, \CPOrdered{\Write{z}{1}}{\Write{z}{2}} because of a \CP ordering
that has not yet been established when \Write{z}{2} executes.}
\label{fig:tricky-true-ruleb}
\end{figure}

==> prior_instance_example.tex <==
%auto-ignore
\begin{figure*} 
\centering 
\begin{tabular}{lllll} 
Thread 1 & Thread 2 & Thread 3 & Thread 4 & Lockset After \\\hline 
\Write{x}{1} &&&& \\
\Acquire{m}{1} &&&& \\
\Release{m}{1} &&&& \\
\Acquire{o}{1} &&&& \\
\Release{o}{1} &&&& \\
\Acquire{q}{1} &&&& \\
\Write{qV}{1} &&&& \\
\Release{q}{1} &&&& \\
& \Acquire{o}{2} &&& \\
& \Acquire{l}{1} &&& \\
& \Release{l}{1} &&& \\
&&& \Acquire{l}{2} & \\
&&& \Release{l}{2} & \\
& \Acquire{p}{1} &&& \\
& \Release{p}{1} &&& \\
&& \Acquire{m}{2} && \\
&& \Acquire{r}{1} && \\
&& \Release{r}{1} && \\ 
&& \Acquire{p}{2} && \\
&& \Release{p}{2} && \\
&& \Release{m}{2} && \\
&&& \Acquire{r}{2} & \\
&&& \Release{r}{2} & \\
&&& \Write{x}{2} & \\
& \Acquire{d}{1} &&& \\
& \Write{dV}{1} &&& \\
& \Release{d}{1}\tikzmark{1} &&& \\
&&& \Acquire{l}{3} & \\
&&& \Acquire{r}{3} & \\
&&& \Release{r}{3} & \\
&&& \tikzmark{2}\Acquire{d}{2} & \\
&&& \Write{dV}{2} & \\
&&& \Release{d}{2} & \\
&&& \Release{l}{3} & \\
& \Release{o}{2} &&&
\end{tabular}

\link{1}{2}

\caption{A racy example on variable \code{x}. Current algorithms will add
\CPThread{T4} to \CPLockSet{x}{1} because $\HBLock{l}{1} \in \HBLockSet{x}{1},
\PCPThread{T4}{l}{} \in \PCPLockSet{x}{1}, \text{ and } \CPThread{T4} \in
\CPLockSet{l}{1}$}
\end{figure*}

==> resultMacros.tex <==
%auto-ignore
\newcommand{\RaptorReadEvents}{0}
\newcommand{\RaptorWriteEvents}{10}
\newcommand{\RaptorAcquireEvents}{10}
\newcommand{\RaptorReleaseEvents}{10}
\newcommand{\RaptorTotalEvents}{30}

==> rule-b-complex-example.tex <==
%auto-ignore
\begin{figure*}
\centering
\begin{tabular}{llllll} 
Thread 1 & Thread 2 & Thread 3 & Thread 4 & Thread 5 & Lockset After \\\hline 
\Write{x}{1} & & & & & \\
\Acquire{o}{1} & & & & & \\
\Release{o}{1} & & & & & \\
\Acquire{t}{1} & & & & & \\
\Release{t}{1} & & & & & \\
& \Acquire{t}{2} & & & & \\
& \Release{t}{2} & & & & \\
& \Acquire{m}{1} & & & & \\ 
& \Release{m}{1} & & & & \\
& \Acquire{q}{1} & & & & \\
& \Write{y}{1} & & & & \\
& \Release{q}{1}\tikzmark{1} & & & & \\
& & \Acquire{o}{2} & & & \\ 
& & \Acquire{p}{1} & & & \\
& & \Release{p}{1} & & & \\
& & & \Acquire{m}{2} & & \\
& & & \Acquire{r}{1} & & \\
& & & \Release{r}{1} & & \\
& & & \Acquire{p}{2} & & \\
& & & \Release{p}{2} & & \\ 
& & & \Release{m}{2} & & \\
& & & & \Acquire{r}{2} & \\
& & & & \Release{r}{2} & \\  
& & & & \Write{x}{2} & \\
& & \tikzmark{2}\Acquire{q}{2} & & & \\
& & \Write{y}{2} & & & \\
& & \Release{q}{2} & & & \\
& & \Release{o}{2} & & & \\

\end{tabular} 

\link{1}{2}

% \mike{Does the algorithm handle this example execution? In particular, when
% \code{T3} unlocks \HBLock{m}{2}, $\code{T3} \notin \CPLockSet{x}{}$, \ie, it's not yet known that there's a CP relationship from \code{x} to the current program point,
% so the algorithm won't/can't transfer CP from the release of \HBLock{m}{2} to the acquire of \HBLock{m}{2}.}
% 
% \jake{First off, I don't believe the current algorithm can handle a situation
% like this. What I'm seeing is a lack of communication between 'dummy'
% locksets. For this example a 'dummy' lockset for \HBLock{m}{2} needs to
% understand that the HB edge from \Release{p} by \code{T2} to \Acquire{p} by
% \code{T3} can become a CP edge since it is a nested lock of a currently held
% lock \code{o}. Now if the critical section on \HBLock{m}{2} (or more
% specifically \Acquire{p} by \code{T3}) occurred after the \Release{o} by
% \code{T2}, CP would be established to the \Acquire{p} by \HBLockSet{o}{1}
% and then \Release{m} by T3 would be CP ordered in which \CPLockSet{x}{}
% would inherit \HBLockSet{m}{2} and problem solved! But due to the lazy CP edge,
% the \HBLockSet{m}{2} must wait for \HBLockSet{o}{1} to deteremine if \Release{p}
% \HBRelation \Acquire{p} is really \Release{p} \CPRelation \Acquire{p}. So the
% algorithm needs to be able to handle this.}
% 
% \mike{An idea for a new direction: Instead of having dummy locksets, add a new
% kind of entry to \emph{variable} locksets: a HB order that's CP if and only if
% CP is established on a lock. For example, $\HBLock{p}{v}:\HBLock{m}{w} \in
% \mathit{PCP}(\code{x})$ (PCP = ``possibly CP'') means that \code{x} is
% \emph{HB}-ordered to \code{p}---and it's \emph{CP}-ordered to \code{p} if/when
% it becomes CP-ordered with \code{m}. (I'm not sure about whether \code{p} and/or
% \code{m} actually need versions.) This dependent property propagates; for
% example, if a thread \code{T} acquires \code{p}, then the algorithm would add
% $\code{T}:\HBLock{m}{w}$ to $\mathit{PCP}(\code{x})$.
% \medskip\\
% Whether or not that's a good idea, at this point I suggest that it would help to
% add to the paper several of the complex Rule (b) examples that have been
% floating around (or make up new ones as needed).}
% \mike{Following up on that, and based on the next two examples, I think the idea may work with the
% following modifications. (1) Add a PCP to each lockset as described above.
% (2) Keep a lockset for a dummy access at the beginning of each critical section.
% The algorithm uses this dummy lockset in order to handle the actions (acquire, release, write) inside of critical sections:
% essentially, the information in the dummy lockset is ``passed on'' to locksets that get updated by these actions.
% \medskip\\
% That may not make sense. I can describe in person.}
% 
% \mike{Following up on your ``Don't be fooled into Rule (b)'' example, I think a
% similar issue exists in this example if we switch \code{T1}'s critical sections
% on \code{o} and \code{m}. In that case, there's a CP-race. So the algorithm
% needs to differentiate those two cases somehow.}

\caption{Rule (b) makes things complex.}
\end{figure*}

 
\begin{figure*}
\centering
\begin{tabular}{llll} 
Thread 1 & Thread 2 & Thread 3 & Lockset After \\\hline 
\Acquire{m}{1} & & & \\
\Acquire{p}{1} & & & \\
\Release{p}{1} & & & \\
& \Acquire{p}{2} & & \\
& \Release{p}{2} & & \\
& \Acquire{n}{1} & & \\
& \Write{y}{1} & & \\
& \Release{n}{1}\tikzmark{1} & & \\
& & \tikzmark{2}\Acquire{n}{2} & \\
& & \Write{y}{2} & \\
& & \Release{n}{2} & \\
\Write{x}{1} & & & \\
\Release{m}{1} & & & \\
& & \Acquire{m}{2} & \\
& & \Release{m}{2} & \\
& & \Write{x}{2} &
\end{tabular}

\link{1}{2}

\caption{Rule (b) gets going before there are any accesses to \code{x}.}
\end{figure*} 


% \begin{figure*} 
% \centering 
% \begin{tabular}{lllll} 
% Thread 1 & Thread 2 & Thread 3 & Thread 4 & Lockset After \\\hline 
% \Write{z}{1} & & & & \\
% \Acquire{q}{1} & & & & \\
% \Release{q}{1} & & & & \\
% & \Acquire{q}{2} & & & \\
% & \Release{q}{2} & & & \\
% \Acquire{m}{1} & & & & \\
% \Release{m}{1} & & & & \\
% & \Sync{n}{1}\tikzmark{1} & & & \\
% & & \Acquire{m}{2} & & \\
% & & \Acquire{o}{1} & & \\
% & & \Release{o}{1} & & \\
% & & & \Acquire{o}{2} & \\
% & & & \Release{o}{2} & \\
% & & & \Write{z}{2} & \\
% & & \tikzmark{2}\Sync{n}{2} & & \\
% & & \Release{m}{2} & & 
% \end{tabular}
% 
% \link{1}{2}
% % \link{1}{2}{12}{-5}{-19}{3}
% 
% \caption{Don't be fooled into Rule (b). \Acquire{m}{1} $\not\CPRelation$ \Release{m}{2}.}
% \label{fig:tricky-false-ruleb}
% \end{figure*}

% \begin{figure*}
% \centering
% \small
% \begin{tabular}{lllll}
% Thread 1 & Thread 2 & Thread 3 & Thread 4 & Lockset After \\\hline
% \Write{x}{} & & & & \HBLockSet{x}{} = \{\HBThread{T1}\} \\
% \Acquire{s}{1} \VCOp{(1,0,0,0)} & & & & \\
% \Release{s}{} & & & & \HBLockSet{x}{} = \{\HBThread{T1}, \VCHBLock{s}{1}{T1(1,0,0,0)}\} \\
% & \Acquire{s}{2} \VCOp{(1,2,0,0)} & & & \HBLockSet{x}{} = \{\HBThread{T1}, \HBThread{T2}, \VCHBLock{s}{1}{T1(1,0,0,0)}\} \\
% & \Release{s}{} & & & \\
% & \Acquire{m}{3} \VCOp{(1,3,0,0)} & & & \HBLockSet{x}{} = \{\HBThread{T1}, \HBThread{T2}, \VCHBLock{s}{1}{T1(1,0,0,0)}, \\
% & & & & \VCHBLock{m}{3}{T2(1,3,0,0)}\} \\
% & \Release{m}{} & & & \\
% \Acquire{o}{4} \VCOp{(4,0,0,0)} & & & & \HBLockSet{x}{} = \{\HBThread{T1}, \HBThread{T2}, \VCHBLock{s}{1}{T1(1,0,0,0)}, \\
% & & & & \VCHBLock{m}{3}{T2(1,3,0,0)}, \VCHBLock{o}{4}{T1(4,0,0,0)}\}\\
% \Release{o}{} & & & & \\ 
% \Acquire{q}{5} \VCOp{(5,0,0,0)} & & & & \HBLockSet{x}{} = \{\HBThread{T1}, \HBThread{T2}, \VCHBLock{s}{1}{T1(1,0,0,0)}, \\
% & & & & \VCHBLock{m}{3}{T2(1,3,0,0)}, \VCHBLock{o}{4}{T1(4,0,0,0)}, \VCHBLock{q}{5}{T1(5,0,0,0)}\}\\
% \Release{q}{} & & & & \\
% & \Acquire{q}{6} \VCOp{(5,6,0,0)} & & & \\
% & \Write{y}{} & & & \HBLockSet{y}{} = \{\HBThread{T2}, \VCLSLock{q}{6}{T2(5,6,0,0)}\} \\
% & \Release{q}{}\tikzmark{1} & & & \\
% & & \Acquire{o}{7} \VCOp{(4,0,7,0)} & & \HBLockSet{x}{} = \{\HBThread{T1}, \HBThread{T2}, \HBThread{T3}, \VCHBLock{s}{1}{T1(1,0,0,0)}, \\
% & & & & \VCHBLock{m}{3}{T2(1,3,0,0)}, \VCHBLock{o}{4}{T1(4,0,0,0)}, \VCHBLock{q}{5}{T1(5,0,0,0)}\}\\
% & & \Acquire{p}{8} \VCOp{(4,0,8,0)} & & \HBLockSet{x}{} = \{\HBThread{T1}, \HBThread{T2}, \HBThread{T3}, \VCHBLock{s}{1}{T1(1,0,0,0)}, \\
% & & & & \VCHBLock{m}{3}{T2(1,3,0,0)}, \VCHBLock{o}{4}{T1(4,0,0,0)}, \VCHBLock{q}{5}{T1(5,0,0,0)}, \\
% & & & & \VCHBLock{p}{8}{T3(4,0,8,0)}\}\\
% & & & & \PCPLockSet{x}{} = \{\PCPLock{p}{8}{o}{7}\}\\
% & & \Release{p}{} & & \\
% & & & \Acquire{m}{9} \VCOp{(1,3,0,9)} & \HBLockSet{x}{} = \{\HBThread{T1}, \HBThread{T2}, \HBThread{T3}, \HBThread{T4}, \VCHBLock{s}{1}{T1(1,0,0,0)}, \\
% & & & & \VCHBLock{m}{3}{T2(1,3,0,0)}, \VCHBLock{o}{4}{T1(4,0,0,0)}, \VCHBLock{q}{5}{T1(5,0,0,0)}, \\
% & & & & \VCHBLock{p}{8}{T3(4,0,8,0)}\}\\
% & & & \Acquire{r}{10} \VCOp{(1,3,0,10)} & \HBLockSet{x}{} = \{\HBThread{T1}, \HBThread{T2}, \HBThread{T3}, \HBThread{T4}, \VCHBLock{s}{1}{T1(1,0,0,0)}, \\
% & & & & \VCHBLock{m}{3}{T2(1,3,0,0)}, \VCHBLock{o}{4}{T1(4,0,0,0)}, \VCHBLock{q}{5}{T1(5,0,0,0)}, \\
% & & & & \VCHBLock{p}{8}{T3(4,0,8,0)}, \VCHBLock{r}{10}{T4(1,3,0,10)}\}\\
% & & & & \PCPLockSet{x}{} = \{\PCPLock{p}{8}{o}{7}, \PCPLock{r}{10}{m}{9}\}\\
% & & & \Release{r}{} & \\
% & & & \Acquire{p}{11} \VCOp{(4,3,8,11)} & \PCPLockSet{x}{} = \{\PCPLock{p}{8}{o}{7}, \PCPLock{r}{10}{m}{9}, \\
% & & & & \PCPLock{p}{11}{m}{9}, \PCPLock{T4}{}{o}{7}\}\\
% & & & \Release{p}{} & \\
% & & & \Release{m}{} & \PCPLockSet{x}{} = \{\PCPLock{p}{8}{o}{7}, \PCPLock{T4}{}{o}{7}\}\\
% & \Acquire{r}{12} \VCOp{(5,12,0,10)} & & & \\
% & \Release{r}{} & & & \\
% & \Write{x}{} & & & $\HBLockSet{x}{`} \leftarrow \HBLockSet{x}{}$\\
% & & & & $\PCPLockSet{x}{`} \leftarrow \PCPLockSet{x}{}$\\
% & & & & $\PCPLockSet{x}{} \leftarrow \emptyset$\\
% & & & & \HBLockSet{x}{} = \{\HBThread{T2}\}\\
% & & \tikzmark{2}\Acquire{q}{13} \VCOp{(5,6,13,0)} & & \PCPLockSet{x}{'} = \{\PCPLock{p}{8}{o}{7}, \PCPLock{T4}{}{o}{7}, \\
% & & & & \PCPLock{q}{13}{o}{7}\}\\
% & & & & \HBLockSet{y}{} = \{\HBThread{T2}, \HBThread{T3}, \VCLSLock{q}{6}{T2(5,6,0,0)}\} \\  
% & & \Write{y}{} & & Check: \VCHBLock{o}{4}{T1(4,0,0,0)} \HBRelation \VCHBLock{q}{6}{T2(5,6,0,0)} \\
% & & & & Giving $4 < 5$. \\ 
% & & & & \CPLockSet{x}{`} = \{\CPThread{T3}, \CPThread{T4}, \CPLock{p}, \CPLock{q}\}\\
% & & & & $\PCPLockSet{x}{`} \leftarrow \emptyset$\\
% & & & & \HBLockSet{y}{} = \{\HBThread{T3}, \VCLSLock{q}{13}{T3(5,6,13,0)}, \VCLSLock{o}{7}{T3(4,0,7,0)}\}\\
% & & \Release{q}{} & & \\
% & & \Release{o}{} & & \CPLockSet{x}{`} = \{\CPThread{T3}, \CPThread{T4}, \CPLock{p}, \CPLock{q}, \CPLock{o}\}\\
% & & & & Race on x since $\PCPLockSet{x}{`} \leftarrow \emptyset$ \\ 
% & & & & and \CPThread{T2} $\notin$ \CPLockSet{x}{`}
% \end{tabular}
% 
% \link{1}{2} 
% 
% \caption{Slightly more complex rule b. x is racy even though q is CP ordered if
% the lock f is CP ordered. This example excludes 'dummy' lockset since it is not used.}
% \label{Fig:complex-racy-rule-b-example}
% \end{figure*}

% Comments about Figure~\ref{Fig:complex-racy-rule-b-example}:
% \jake{On \Write(y) by \code{T3}. Since CP is established while \HBLock{o}{7} is still held, the \PCPLockSet{x}{`} wants to check if \code{x`} has a prior
% \HBLock{o}{} \HBRelation \HBLock{o}{7}. If so, then all dependencies on \HBLock{o}{7} are added to \CPLockSet{x}{`} and removed from PCP.}
% \jake{At \Release{o} by \code{T3}. If \PCPLockSet{x}{`} has no more dependencies and no CP was established to the thread the lazy
% access was first accessed from, the lazy race is a true race. The CP established thread must be from the PCP lockset and once
% a lazy race is discovered, no new threads can be added to the PCP set. Since a situation such as switching x before a(r)/r(r) 
% could give a false CP edge to the lazy race. }
% \jake{\PCPLockSet{x}{} would gain \PCPLock{m}{9}{o}{7} at the \Release{m} by
% \code{T4} because \HBLock{p}{8} has an earlier version than \HBLock{p}{11}. Therefore, \HBLock{p}{8} \HBRelation \HBLock{p}{11} 
% which implies \Acquire{o}{7} \HBRelation \Release{m} by \code{T4}. But, since
% \HBLock{m}{3} $\not$\HBRelation \HBLock{o}{4}, no future established CP edge
% could establish a CP edge from \HBLock{m}{3} to \HBLock{m}{9}. Therefore, at the
% \Release{m} by \code{T4}, all dependent locks are removed from the PCP set.
% This also brings up an interesting point that if \Acquire{p}{8} was moved below
% \Acquire{p}{11} then \Acquire{o}{7} $\not$\HBRelation \Release{m} by \code{T4}.
% So CP does still suffer the same issue of needing to explore different interleavings leading to switching HB edges in order to discover all predicitable races.}
% \jake{At the \Acquire{q}{7} I am unsure if the update
% to VC for \code{T3} is correct. To update it, goldCP is using the stored state
% of \HBLock{q}{4}. This choice is made because no event after \HBLock{q}{4} in
% \code{T2} has a HB relation to \Acquire{q}{7}.} 
% \jake{Side Note: Using order in \HBLockSet{x}{} the element \VCHBLock{m}{3}{T2(1,3,0,0)} can be reduced to \VCHBLock{m}{3}{(1,3,0,0)}. 
% So \HBLockSet{x}{} = \{\HBThread{T1}, \VCHBLock{m}{3}{(1,3,0,0)}, \HBThread{T2}\} would mean \HBLock{m}{3} was acquired in \code{T1} where
% \HBLockSet{x}{} = \{\HBThread{T1}, \HBThread{T2}, \VCHBLock{m}{3}{(1,3,0,0)}\} would mean \HBLock{m}{3} was acquired in \code{T2}}

% Can you show how this case is handled? Keeping in
% mind, the algorithm should also be able to handle the correct case of
% acq(f)/rel(f) by T2 becoming a sync(f) and the sync(f) by T1 becoming a
% acq(f)/rel(f). I am mostly confused on how to handle the same lock needing the
% information along two separate paths. Seems like a lock f element is needed for
% both T1 and T2.}

\begin{figure*} 
\centering 
\begin{tabular}{lllll} 
Thread 1 & Thread 2 & Thread 3 & Thread 4 & Lockset After \\\hline 
\Write{x}{1} & & & & \\
\Acquire{q}{1} & & & & \\
\Write{y}{1} & & & & \\
\Release{q}{1}\tikzmark{1} & & & & \\
\Acquire{m}{1} & & & & \\
\Release{m}{1} & & & & \\
& & \Acquire{m}{2} & & \\
& & \Acquire{r}{1} & & \\
& & \Release{r}{1} & & \\
& \tikzmark{2}\Acquire{q}{2} & & & \\
& \Write{y}{2} & & & \\
& \Release{q}{2} & & & \\
& \Acquire{t}{1} & & & \\
& \Release{t}{1} & & & \\
\Acquire{t}{2} & & & & \\
\Release{t}{2} & & & & \\
\Acquire{b}{1} & & & & \\
\Write{y}{3} & & & & \\
\Release{b}{1}\tikzmark{3} & & & & \\
& \tikzmark{4}\Acquire{b}{2} & & & \\
& \Write{y}{4} & & & \\
& \Release{b}{2} & & & \\
& & \Acquire{t}{3} & & \\
& & \Release{t}{3} & & \\
& & \Release{m}{2} & & \\
& & & \Acquire{r}{2} & \\
& & & \Release{r}{2} & \\ 
& & & \Write{x}{2} & 
\end{tabular}

\link{1}{2}
\link{3}{4}
  
\caption{Example to make it hard to determine if \Acquire{m}{1} \CPRelation \Release{m}{2} because we need to know if
\Acquire{m}{1} \HBRelation \Release{q}{1}}
\end{figure*}

\begin{figure*} 
\centering 
\begin{tabular}{lllll} 
Thread 1 & Thread 2 & Thread 3 & Thread 4 & Lockset After \\\hline 
\Write{x}{1} & & & & \\
\Acquire{w}{1} & & & & \\
\Release{w}{1} & & & & \\
& & & \Acquire{w}{2} & \\
& & & \Release{w}{2} & \\
& & & \Acquire{t}{1} & \\
& & & \Release{t}{1} & \\
\Acquire{m}{1} & & & & \\
\Release{m}{1} & & & & \\
& & \Acquire{m}{2} & & \\
& & \Acquire{r}{1} & & \\
& & \Release{r}{1} & & \\
\Acquire{s}{1} & & & & \\
\Release{s}{1} & & & & \\
& & & \Acquire{s}{2} & \\
& & & \Release{s}{2} & \\
& & & \Acquire{q}{1} & \\
& & & \Write{y}{1} & \\
& & & \tikzmark{1}\Release{q}{1} & \\
& \Acquire{q}{2}\tikzmark{2} & & & \\
& \Write{y}{2} & & & \\
& \Release{q}{2} & & & \\
& \Acquire{t}{2} & & & \\
& \Release{t}{2} & & & \\
& & \Acquire{t}{3} & & \\
& & \Release{t}{3} & & \\
& & \Release{m}{2} & & \\
& & & \Acquire{r}{2} & \\
& & & \Release{r}{2} & \\
& & & \Write{x}{2} &
\end{tabular}

\link{1}{2}
  
\caption{Another example needing to distinguish the difference of having the \Acquire{s}{1} in which no race on x exists and not having the
\Acquire{s}{1} which can not CP order the second access to x}
\end{figure*}

% \begin{figure*} 
% \centering 
% \begin{tabular}{lllll} 
% Thread 1 & Thread 2 & Thread 3 & Thread 4 & Lockset After \\\hline
% \Write{x}{1} & & & & \\ 
% \Acquire{m}{1} & & & & \\
% \Release{m}{1} & & & & \\
% \Acquire{o}{1} & & & & \\
% \Release{o}{1} & & & & \\
% \Acquire{q}{1} & & & & \\
% \Write{y}{1} & & & & \\
% \Release{q}{1}\tikzmark{1} & & & & \\
% & \Acquire{o}{2} & & & \\
% %& \Acquire{p}{1} & & & \\
% %& \Release{p}{1} & & & \\
% & & \Acquire{m}{2} & & \\
% & & \Acquire{p}{1} & & \\
% & & \Release{p}{1} & & \\
% %& \Write{x}{1} & & & \\
% & \Acquire{r}{1} & & & \\
% & \Release{r}{1} & & & \\ 
% & & \Acquire{r}{2} & & \\
% & & \Release{r}{2} & & \\
% & & \Release{m}{2} & & \\
% & & & \Acquire{p}{2} & \\
% & & & \Release{p}{2} & \\
% %& & & \Acquire{m}{3} & \\
% %& & & \Release{m}{3} & \\
% & & & \Write{x}{2} & \\
% & \tikzmark{2}\Acquire{q}{2} & & & \\
% & \Write{y}{2} & & & \\
% & \Release{q}{2} & & & \\
% & \Release{o}{2} & & &
% \end{tabular}
% 
% \link{1}{2}
%   
% \caption{Example to show how a 'dummy' lockset and a PCP set need to work together.}
% \label{fig:ruleb-transfer-needed}
% \end{figure*}


\begin{figure*} 
\centering 
\begin{tabular}{lllll} 
Thread 1 & Thread 2 & Thread 3 & Lockset After \\\hline 
& \Acquire{m}{1} & & \\
& \Acquire{n}{1} & & \\
& \Write{y}{1} & & \\
& \Release{n}{1}\tikzmark{3} & & \\
\Write{x}{1} & & & \\
\Acquire{o}{1} & & & \\
\Release{o}{1} & & & \\
& \Acquire{o}{2} & & \\
& \Release{o}{2} & & \\
\Acquire{q}{1} & & & \\
\Write{z}{1} & & & \\
\Release{q}{1}\tikzmark{1} & & & \\
& \tikzmark{2}\Acquire{q}{2} & & \\
& \Write{z}{2} & & \\
& \Release{q}{2} & & \\
& \Release{m}{1} & & \\
& & \tikzmark{4}\Acquire{n}{2} & \\
& & \Write{y}{2} & \\
& & \Release{n}{2} & \\
& & \Acquire{m}{2} & \\
& & \Release{m}{2} & \\
& & \Write{x}{2} & 
\end{tabular}

\link{1}{2}
\link{3}{4}

\caption{Complicates the distinction between rule b for lock \code{o} and rule b for lock \code{m}}
\end{figure*}

